An Improved Lower Bound for Matroid Intersection Prophet Inequalities

We consider prophet inequalities subject to feasibility constraints that are the intersection of $q$ matroids. The best-known algorithms achieve a $\Theta(q)$-approximation, even when restricted to instances that are the intersection of $q$ partition matroids, and with i.i.d.~Bernoulli random variables. The previous best-known lower bound is $\Theta(\sqrt{q})$ due to a simple construction of [Kleinberg-Weinberg STOC 2012] (which uses i.i.d.~Bernoulli random variables, and writes the construction as the intersection of partition matroids). We establish an improved lower bound of $q^{1/2+\Omega(1/\log \log q)}$ by writing the construction of [Kleinberg-Weinberg STOC 2012] as the intersection of asymptotically fewer partition matroids. We accomplish this via an improved upper bound on the product dimension of a graph with $p^p$ disjoint cliques of size $p$, using recent techniques developed in [Alon-Alweiss European Journal of Combinatorics 2020].

==> Files/aa19.tex <==
%!TeX root = ../main.tex
%!TEX root = ../main.tex 

\section{Proof of the main theorem}
Consider the following bipartite graph $H=(L,R)$:
\begin{itemize}
    \item $L$ is the set of all permutations on $\ell$ elements.
    \item $R$ is the set of all balanced words in $\zp^\ell$.
    \item $\pi\in L$ is adjacent to $w\in R$ if and only if $\pi(w)$ is special.
\end{itemize}
Let $d_L$ denote the degree of a vertex in $L$ and $d_R$ denote the degree of a vertex in $R$ (by symmetry, every vertex in $L$ (respectively $R$) has the same degree). Observe that $d_L$ is the total number of special balanced words. We have $|L|=\ell!$, $|R|< (p-1)^\ell$ and $d_L > 2^\ell/\ell^{p/2}$. Using the fact that $d_R = \frac{|L|}{|R|} \cdot d_L$, we get that $d_R\ge \log 2|R|$. Hence by \autoref{lem:bp}, we conclude that we can partition $R=S_1\sqcup S_2\sqcup \dots$ such that each $|S_i|>2^\ell/\ell^{p}$ and for every $i$, there exists $\pi_i$ such that for every $s\in S_i$, $\pi_i(s)$ is a special balanced word.

\paragraph{Proof sketch}
Observe that the code of all special balanced words has $+1$ and $-1$ as shattered elements. Let $\alpha$ be a primitive root modulo $p$. The main idea is to amplify the shattered set in $r$ steps to $\{\pm \alpha^b\}$ for $0\le b < 2^r$ such that the total number of codewords is still $(2-o(1))^\ell$. Thus, after roughly $O(\log p)$ iterations, we have a code with $\zp^*$ as shattered set. In the end, we can add an extra coordinate of $0$ to every codeword to get $\zp$.

\subsection{The iterative procedure}

We first describe the iterative procedure in detail here and defer the analysis of parameters to the next subsection.

Let $C_r,N_r,\ell_r,s_r$  respectively denote the code, size of the code, the length of the code and the size of the shattered set at the end of $r$ steps. Let $z$ be a parameter that will be fixed later. Fix $\alpha$ to be a primitive root modulo $p$. Initial conditions: We will fix $\ell_0$ later as a function of $p$. $C_0$ is the set of all special balanced codewords in $\zp^{\ell_0}$. Clearly, the code has has $+1$ and $-1$ as shattered elements and hence $s_0 = 2$.

\paragraph{First step}
Let $B_0$ denote the set of all balance words in $\zp^{\ell_0}$. Let $B_0=S_{1}\sqcup S_{2}\sqcup \dots$ such that each $|S_{i}|>(2-o(1))^{\ell_0}$ and for every $i$, there exists $\pi_i$ such that for every $s\in S_{i}$, $\pi_i(s)\in C_0$, i.e., $\pi_i(s)$ is a special balanced word. Let $\ell_1 = z\ell_0$. We first construct a family of codes $\Cc_1=\{C(w,y)\subseteq \zp^{\ell_1}:w,y\in B_0\}$ and then choose $C_1$ to be the largest code in this family. The following is the description of code $C(w,y)\subseteq \zp^{\ell_1}$: $(x_1,x_2,\dots,x_z)\in C(w,y)$ if and only if 
\begin{enumerate}
    \item $x_i \in B_0$, for every $i$.
    \item For all $i<z$, if $x_i\in S_j$, then $x_{i+1}\in \alpha S_j$, i.e., $\alpha^{-1} x_{i+1}\in S_j$.
    \item $x_1 = w$ and $x_z=y$.
\end{enumerate}
\begin{lemma}
Every code in $\Cc_1$ has $\{\pm1,\pm\alpha\}$ as shattered elements.
\end{lemma}
\begin{proof}
Consider two arbitrary codewords $(x_1,x_2,\dots,x_z)$ and $(x'_1,x'_2,\dots,x'_z)$. We have $x_1=x'_1$ and $x_z=x'_z$. Let $i$ denote the smallest index such that $x_i\ne x'_i$ and $j$ denote the largest index such that $x_j\ne x'_j$. We have $x_{i-1}=x'_{i-1}\in S_k$, for some $k$. Hence $\alpha^{-1}x_i\neq \alpha^{-1}x'_i \in S_k $ and therefore, $\alpha^{-1}(x_i-x'_i)$ contains $\pm1$ and hence, $(x_i-x'_i)$ contains $\pm \alpha$. We have $x_{j+1}=x'_{j+1}\in \alpha S_l$, for some $l$. This implies that $x_j,x'_j\in S_l$ and hence $(x_j-x'_j)$ contains $\pm 1$. This shows that $\{\pm1,\pm\alpha\}$ are shattered elements.
\end{proof}

We will iteratively construct a code such that $C_r$ has $\{\pm \alpha^i: 0\le i < 2^r\}$ as shattered elements.

\paragraph{$r$-th step}
We will construct a code such that $N_r \approx N_{r-1}^z$, $\ell_r = z\cdot \ell_{r-1}$, and $s_r = 2\cdot s_{r-1}$. Let $B_{r-1}$ denote the set of all balanced words in $\zp^{\ell_{r-1}}$. Let $B_{r-1}=S_{1}\sqcup S_{2}\sqcup \dots$ such that each $|S_{i}|>(2-o(1))^{\ell_{r-1}}$ and for every $i$, there exists $\pi_i$ such that for every $s\in S_{i}$, $\pi_i(s) \in C_{r-1}$ (in \autoref{sec:analysis}, we will later prove that such a partition exists by applying \autoref{lem:bp}). We first construct a family of codes $\Cc_r=\{C(w,y)\subseteq \zp^{\ell_r}:w,y\in B_{r-1}\}$ and then choose $C_r$ to be the largest code in this family.

The following is the description of code $C(w,y)\subseteq \zp^{\ell_r}$: $(x_1,x_2,\dots,x_z)\in C(w,y)$ if and only if 
\begin{enumerate}
    \item $x_i \in B_{r-1}$, for every $i$.
    \item For all $i<z$, if $x_i\in S_j$, then $x_{i+1}\in \alpha^{2^{r-1}} S_j$.
    \item $x_1 = w$ and $x_z=y$.
\end{enumerate}
\begin{lemma}
Every code in $\Cc_r$ has  $\{\pm \alpha^i: 0\le i < 2^r\}$ as shattered elements.
\end{lemma}
\begin{proof}
We will assume by induction that $\Cc_{r-1}$ has $\{\pm \alpha^i: 0\le i < 2^{r-1}\}$ as shattered elements. Consider two arbitrary codewords $(x_1,x_2,\dots,x_n)$ and $(x'_1,x'_2,\dots,x'_n)$. Let $i$ denote the smallest index such that $x_i\ne x'_i$ and $j$ denote the largest index such that $x_j\ne x'_j$. We have $x_{i-1}=x'_{i-1}\in S_k$, for some $k$. Hence $\alpha^{-2^{r-1}}x_i\neq \alpha^{-2^{r-1}}x'_i \in S_k $ and therefore, $\alpha^{-2^{r-1}}(x_i-x'_i)$ contains $\{\pm \alpha^i: 0\le i < 2^{r-1}\}$ and hence, $(x_i-x'_i)$ contains $\{\pm \alpha^i: 2^{r-1}\le i < 2^{r}\}$. We have $x_{j+1}=x'_{j+1}\in \alpha^{2^{r-1}} S_l$, for some $l$. This implies that $x_j,x'_j\in S_l$ and hence $(x_j-x'_j)$ contains $\{\pm \alpha^i: 0\le i < 2^{r-1}\}$. This shows that $\{\pm \alpha^i: 0\le i < 2^{r}\}$ are shattered elements.
\end{proof}

\subsection{Parameter analysis}\label{sec:analysis}
\Vnote{I am not redoing the analysis of [AA20] since by their construction, they require $\ell$ to be at least $p^{O(\log\log p)}$ to get $\zp$ as the shattered set. In this section, I hope to analyse the minimum $z$ required in each step of the iterative process and the best initial $\ell_0$. To apply their construction, we need $\ell_0$ to be a multiple of $p-1$. Their initial $\ell_0 = O(p^2)$. Is such a large $\ell_0$ essential?} 


{\color{blue}{Getting the right parameters: Let $K = p^{1/\log \log p}$ be the number of shattered elements we are targeting after we finish the [AA20] approach. One approach is to start with balanced codewords that are only balanced on the first $K$ elements of $[p-1]$. This allows a smaller value of $\ell_0$.}}

Let us set $\ell_0=p-1$. We have $N_0=|B_0|=(p-1)!$, where $B_0$ is the set of all balanced words in $\zp^{p-1}$. Since we set $C_0$ to be the set of all special balanced codewords in $\zp^{\ell_0}$, we have $N_0=2^{(p-1)/2}$.


We will now determine how large we need $z$ to be and obtain a lower bound on $N_r$. Let us now focus on the $r$-th step. We have $\ell_r = z\cdot \ell_{r-1}$. In order to obtain a precise lower bound on the size of each $S_i$ in the partition of $B_{r-1}$ that we considered, let us construct the following bipartite graph $H(L,R)$:
\begin{enumerate}
    \item $L$ is the set of all permutations on $\ell_{r-1}$ symbols.
    \item $R=B_{r-1}$.
    \item $\pi \in L$ is adjacent to $w\in R$ if and only if $\pi(w)\in C_{r-1}$.
\end{enumerate}

Let $d_L,d_R$ denote the left and right degrees respectively. We have $d_R = \frac{|L|}{|R|}\cdot d_L = \frac{\ell_{r-1}!}{|B_{r-1}|}\cdot |N_{r-1}|$. When is $d_R\ge \log 2|R|$? Applying \autoref{lem:bp}, we can lower bound $|S_i|$ as $|S_i|\ge d_L/(4\log 2|R|) = N_{r-1}/(4\log 2|B_{r-1}|)$.

Ignoring the constant factors, we can bound $N_r$ as 
\[
N_r \ge |S_i|^{z-1}/|R| = N_{r-1}^{z-1}/(|B_{r-1}|\cdot (\log |B_{r-1}|)^{z-1})
\]


{\color{blue}{Even if the above term was as large as $N_{r-1}^{z-1}$ and $N_{r-1}$ was as large as $2^{\ell_{r-1}}$, that would mean that 
\[
N_r \geq N_{r-1}^{z-1} = 2^{\ell_{r-1} \cdot (z-1)} = 2^{z\ell_{r-1} \cdot (1-1/z)}  = 2^{\ell_r \cdot (1-1/z)} = (2^{1 - 1/z})^{\ell_r} .
\]
By Taylor expansion, (click \href{https://www.wolframalpha.com/input/?i=2\%5E\%7B1-x\%7D+taylor}{here}) the base becomes $2 - O(1)/z$ implying that we lose an additive $O(1)/z$ at every step. This means that we can do at most $z$ steps.


Now, note that at the end of $z$ steps the number of codewords is at most $2^{\ell_0 z^z}$. As we want $\ell_0$ to be small and the number to be $p^p$, we would like $z$ to be roughly logarithmic.

}}


\subsection{Our construction: Code of size $p^p$ with $\zp$ as the shattered set and $\ell=o(p^2)$}



Suppose we have a code $\Cc$ with $N \sim 2^{\ell}$ codewords, length $\ell$, and $k$ shattered elements of the form $\{ \alpha^i \mid 0 \leq i < k \}$. Define a related code $\mathcal{D}$ as follows:

\[
\mathcal{D} = \{ C \Vert \alpha^k C \mid C \in \Cc \}
\]

If initially $k = p^{1/\log \log p}$ and $\ell = p\log p$, then after applying this operation $\log p - \log p /\log \log p$ times, we will have $k = p$ and $\ell = p^{2 - 1 /\log \log p}$.

In general, if we start from $\ell = p\log p$, then we'll have $N = p^p$. If we can get there for a certain $k$, then we'd need to do this operation $\log_2(p/k)$ times, which would turn $\ell$ into $\ell \cdot p/k$.

Their operation maintains $N = 2^\ell$ (so we don't need to keep track of this as we go). Their operation, done a total of $r$ times, gives $k=2^r$, and multiplies $\ell$ by $r^r$. 

So in particular, if we start with any initial $\ell$, the blowup in $\ell/k$ is always $\geq 1$, so this means that the absolute best we could hope for (which still might not be achievable) is $\ell p$ (where $\ell$ is the initial $\ell$). 

\Vnote{Moved the previous section 6 to scratch.tex}

























==> Files/lowerbound.tex <==
%!TeX root = ../main.tex 
%!TEX root = ../main.tex



\section{$\zp$-covering families via Concatenation}
\label{sec:lowerbound}


Our proof of~\cref{thm:upperbound} starts from $\Ff_1$, an existing $\mathbb{Z}_{k}$-covering $(\ell_1,k)$-family. Then, we pick a larger $p$ and turn $\Ff_1$ into a $[0, k-1]$-covering $(\ell_2,p)$- family, $\Ff_2$ (\cref{lem:ff2}). Finally, we turn $\Ff_2$ into a $\mathbb{Z}_{p}$-covering $(\ell_3,p)$-family $\Ff_3$ (\cref{thm:upperbound}). In particular, observe that the blowup going from $\Ff_1$ to $\Ff_2$ is always at most $O(\log_2p)$, while the blowup going from $\Ff_2$ to $\Ff_3$ is always at least $\Omega(\log_2 (p))$, and these bounds are tight only when $k = \Theta(p)$. Indeed, for the range of parameters we're most interested in ($N= p^p$), and given the best-known existing constructions ($\ell_1 \approx \log_2 (N)$, but only when $N \geq 2^{p^{5 \log_2 \log_2 p}}$), we have $k = 2^{\Theta(\frac{\log_2 p}{\log_2\log_2 p})}$. Therefore, second step costs a factor of $p \ln(p)/k=\tilde{\Omega}(p)$. This suggests that possible paths towards improvement are (a) finding a better base construction, and (b) improving our second step transitioning from $\Ff_2$ to $\Ff_3$. While (a) is outside the scope of this paper, we spend the rest of this section examining the extent to which (b) might be possible.

In particular, observe that our construction from $\Ff_2$ to $\Ff_3$ proceeds simply by \emph{concatenating} elements of $\Ff_2$ together, multiplied by some scalars. The construction is also black-box with respect to $\Ff_2$: the only fact about $\Ff_2$ that is used is that $\Ff_2$ is $[0, k-1]$-covering.

\begin{definition}[Concatenation Procedure]
A \emph{concatenation procedure} takes as input a non-empty $(\ell,p)$-family $\mathcal{V}$, an integer $z$, and a sequence $(\alpha_1,\ldots, \alpha_z)$, where each $\alpha_j \in \mathbb{Z}_p$. The procedure outputs the largest $\mathbb{Z}_p$-covering $(z\ell,p)$-family $\mathcal{V}'$ that is a subset of the set $\mathcal{W}:=\{(\alpha_1\vec{v}_1,\ldots, \alpha_z \vec{v}_z)\ |\ \vec{v}_j \in \mathcal{V}\ \forall j\}$. 

That is, all elements in $\mathcal{V}'$ must be the concatenation of $z$ elements in $\mathcal{V}$, where the $j^{th}$ concatenated element is scalar-multiplied by $\alpha_j$. Then $\mathcal{V}'$ is the largest such set that is also $\mathbb{Z}_p$-covering.

We say that a concatenation procedure and lower bound on the size of its output is $(z,k,p)$-\emph{agnostic} if the proof relies only on the fact that $\mathcal{V}$ is $T$-covering for some set of size $k$ (and just the fact that $|T| = k$).
\end{definition}

Our procedure to get from $\Ff_2$ to $\Ff_3$ (\cref{thm:upperbound}) is a concatenation procedure, and the proof is agnostic. We now show that agnostic concatenation procedures cannot do much better than ours.


\begin{proposition}\label{prop:concatenation}
Every $(z,k,p)$-agnostic concatenation procedure with $k$ prime and $k \in [3,\frac{p-1}{4}]$ results in a lower bound on $|\mathcal{V}'|$ no better than $|\mathcal{V}|^{\frac{4zk}{p-1}}$.


\end{proposition}

\begin{proof}
Let $\Vv$ be the $[k]$-covering $(\ell_2,p)$-family $\Ff_2$ constructed in the proof of \cref{lem:ff2}. Observe in particular that every coordinate of every vector in $\Ff_2$ lies in $[0,2k] \pmod p$. This immediately implies that for any $\vec{v},\vec{w} \in \Ff_2$ and every coordinate $i$, we have $v_i - w_i \in (-2k,2k) \pmod p$, and in particular there are at most $4k$ possibilities. From this, we further conclude that for all $j$, the range of $\alpha_j \cdot (v_i,w_i)$, where $\vec{v},\vec{w} \in \Ff_2$, also has size at most $4k$. Refer to this set as $S_j$.

Now, this means that there are at most $4zk$ pairs $(g,j)$ where $g \in  \zp\setminus \{0\}$ and $g \in S_j$. In particular, there must exist some $h \in \zp$ that is in at most $4zk/(p-1)$ such pairs. Let $T_h:=\{j\ |\ h \in S_j\}$. 

Now, consider any two elements $\vec{v}:=(\alpha_1 \vec{v}_1,\ldots, \alpha_z \vec{v}_z),\vec{w}:=(\alpha_1\vec{w}_1,\ldots, \alpha_z \vec{w}_z)$ of $\mathcal{V}'$. In order to have $\alpha_j v_{ji} - \alpha_j w_{ji} = h$, we must have $j \in T_h$ (by definition). Moreover, because $h \neq 0 \pmod p$, we must have $\vec{v}_j \neq \vec{w}_j$. In particular, this means that \emph{every two vectors in $\mathcal{V}'$ must differ in at least one coordinate in $T_h$}. There are only $|\mathcal{V}|^{|T_h|}$ such possibilities, implying that $|\mathcal{V}'| \leq |\mathcal{V}|^{|T_h|} = |\mathcal{V}|^{\frac{4zk}{p-1}}$.

Observe that $\Ff_2$ covers a set of size $k$, so any $(z,k,p)$-agnostic concatenation procedure would work starting from $\Ff_2$. We've shown that no lower bound better than $|\mathcal{V}|^{\frac{4zk}{p-1}}$ is possible, and therefore no lower bound better than this is possible from any $(z,k,p)$-agnostic concatenation procedure.
\end{proof}

\cref{prop:concatenation} establishes that significant quantitative improvements on our concatenation procedure are not possible. Indeed, it follows from \cref{prop:concatenation} that to preserve the size of the family, $z$ must be at least $\frac{p-1}{4k}$. Hence, the blowup in length going from $\Ff_2$ to $\Ff_3$ is optimal up to a $\Theta(\log_2 (p))$ factor.
Therefore, the possible avenues towards better bounds on $\AAM(p,p^p)$ using a similar approach are: (a) a better starting point than~\cref{thm:aa20}, or (b) a non-agnostic concatenation procedure.


%We claim that there exists a subset $S'\subseteq \zp$ of size at most $4k$ such that for every pair of vectors $\vec{v},\vec{w}\in \Vv$, for all $i\in [\ell_2]$, $v_i-w_i \mod p\in S'$. Before proving the claim, we prove the lemma using this claim. Let $\Vv'$ denote the output of the concatenation procedure on input $\Vv$. Since $\Vv'$ is $\zp$-covering, we have $\zp = \alpha_1 S' \cup \alpha_2 S' \cdots \cup \alpha_{\len*{ \vec{\alpha} }} S'$. Hence, there exists $g\in \zp$ that is contained at most $\frac{\len*{ \vec{\alpha} } \cdot 4k}{p-1}$ of the $\alpha_i S'$ sets. Let $I_g = \{i\in [\len*{ \vec{\alpha} }] \mid g\in \alpha_i S' \} $. For any pair of vectors $\paren*{ \alpha_1 \vec{v}_1, \alpha_2 \vec{v}_2, \cdots, \alpha_{ \len*{ \vec{\alpha} } } \vec{v}_{ \len*{ \vec{\alpha} } } } \ne  \paren*{ \alpha_1 \vec{w}_1, \alpha_2 \vec{w}_2, \cdots, \alpha_{ \len*{ \vec{\alpha} } } \vec{w}_{ \len*{ \vec{\alpha} } } } \in \Vv'$, there must exist some $j\in I_g$ such that $\vec{v}_j \neq \vec{w}_j$. Since $|I_g|\le \frac{\len*{ \vec{\alpha} } \cdot 4k}{p-1}$, we conclude that $|\Vv'|\le |\Vv|^{\frac{\len*{ \vec{\alpha} } \cdot 4k}{p-1}}$. Let us now prove the claim. Observe that any $\vec{v}\in \Vv'$ is contained in $[0,2k-1]^{\ell_2}$. Hence for any pair of vectors $\vec{v},\vec{w}\in \Vv$, for all $i\in [\ell_2]$, $v_i-w_i \mod p \in (-2k ,2k)$. This completes the proof.

%Let $\Ff_0$ be an $(\ell_0,p)$-Family that is $S$-covering for $S\subseteq \zp$. Let $\Ff$ be an $(\ell,p)$-Family that is $\zp$-covering. Say $\ell = z \ell_0$ and there exists $\alpha_1,\dots,\alpha_z \in \zp$ such that every $\vec{u}\in \Ff$ is of the form $\vec{u} = (\alpha_1 \vec{u_1},\dots,\alpha_{z} \vec{u_z})$ for $\vec{u_1},\dots,\vec{u_z}\in \Ff_0$. The following lemma bounds the maximum number of vectors in $\Ff$.

%\begin{lemma}[Upper bound on the size of a concatenated family]
%For families $\Ff,\Ff_0$ that satisfy the conditions stated above, we have 
%\[|\Ff|\le |\Ff_0|^{\frac{z |S|}{p-1}}\, .\]
%\end{lemma}
%\Vnote{Not sure if this is lemma is correct as stated. What's the issue? In my informal note, I made the assumption that every pair of codewords shatters exactly the set $S$. But this is not true in general. A given pair of codewords could shatter a superset of $S$, even $\zp$. $S$ is only the intersection of all these shattered sets. Not sure if it is still possible to prove the lemma without this assumption. Suggestions for a modified statement that is still interesting?}

%\begin{definition}[Concatenation of vectors]
%We say that an $L$-length vector $\vec{u}$ is a concatenation of vectors from an 
%$(\ell,p)$-Family $\Ff$ if $\ell$ divides $L$ and there exists %$\vec{u_1},\dots,\vec{u_z}\in \Ff$ and $\alpha_1,\dots,\alpha_z \in \zp$ for %$z=L/\ell$ such that  $\vec{u} = (\alpha_1 \vec{u_1},\dots,\alpha_{z} \vec{u_z})$.

%\end{definition}

%\begin{lemma}
%Let $\Ff$ be a $\zp$-covering, $(\ell,p)$-Family such that every $\vec{u}\in \Ff$ is %a concatenation of vectors from an $(\ell_0,p)$-Family $\Ff_0$ that is $S$-covering, %then ...
%\end{lemma}




\iffalse

We fix a prime $p > 0$ and work in the field $\zp$. For $z > 0$, it shall sometimes be convenient to view vectors in $\zp^{z\ell}$ and elements of $\paren*{ \zp^{\ell} }^z$. A concatenation procedure for families is defined by a sequence $\vec{\alpha} \in \zp^*$. It takes as input a non-empty $(\ell, p)$-Family $\mathcal{V}$, for some $\ell > 0$ and acts as follows: First, it constructs an $(\ell \cdot \len*{ \vec{\alpha} }, p)$-Family $\mathcal{W}$ as:
\[
\mathcal{W} = \set*{ \paren*{ \alpha_1 \vec{v}_1, \alpha_2 \vec{v}_2, \cdots, \alpha_{ \len*{ \vec{\alpha} } } \vec{v}_{ \len*{ \vec{\alpha} } } } \mid \vec{v}_1, \vec{v}_2, \cdots, \vec{v}_{ \len*{ \vec{\alpha} } } \in \mathcal{V} } .
\]
Then, it outputs the largest subset $\mathcal{V}' \subseteq \mathcal{W}$ that is $\zp$-covering, breaking ties lexicographically. Such a family always exists as an empty family trivially satisfies \cref{def:covering}.

Consider the concatenation procedure defined by a sequence $\vec{\alpha} \in \zp^*$. For every prime $k\in [3,\frac{p-1}{4}]$, there exists $S\subseteq \zp$ such that $|S|=k$ and an $S$-covering family $\Vv$ such that
\[ \log_{|\Vv|} |\Vv'|\le \frac{\len*{ \vec{\alpha} } \cdot 4k}{p-1}\, ,\] where $\Vv'$ is the output of the concatenation procedure.



\fi







































==> Files/scratch.tex <==
\section{Raghuvansh's thing}

Construction:
\begin{itemize}
    \item Start with a code $C$ of $N$ codewords with length $\ell$ that shatters $\alpha^i$ for all $0 \leq i < k$.
    \item Pick a sequence of $2r$ numbers $a_1,\ldots, a_r, b_1,\ldots, b_r$ such that $a_i\le b_i, \forall i$. \item The level-$i$ codewords will be triples of scaled level-$(i-1)$ codewords. 
    \item There will be $\Theta(N^{2^i})$ codewords in level $i$. 
    \item In particular, the level-$i$ code will proceed as follows:
    \begin{itemize}
        \item Pick a subset of $N^{2^i}$ triples of level-$(i-1)$ codewords, such that for any two distinct triples in the subset, they differ in at least two coordinates. Note that a set of the desired size necessarily exists.
        \item The first coordinate is scaled by $1$, the second by $\alpha^{a_i}$, the third by $\alpha^{b_i}$.
    \end{itemize}
    \item Now, the goal is to figure out whether $\alpha^x$ is shattered. Consider now two codewords from level $r$. 
    
    
\end{itemize}

\Vnote{Issues with the current construction: No unique $Y$ for the entire code. Given any pair of codewords from the final code, we can draw a binary tree like structure where at the root we look at the level-$(r-1)$ codewords where they differ  -  the left child corresponds to the level-$(r-1)$ codeword  with the smallest multiplier (either $1$ or $\alpha^{a_r}$), and then repeat the same as we go down. For every leaf in this tree, we have a corresponding $Y$. For this $Y$, given $x\in \mathbb{Z}_p^*$, there is some $w\in \{0,1\}^r$ such that the subset sum equals $x$. However, this $w$ also roughly tells us the path we take down in the binary tree, and may not be compatible with our initial choice of $Y$. Hence $w$ needs to be determined in an online way. Not clear if there exists a sequence of triples for which we can do this. Another thing that we considered was a code where level-$i$ codewords are quadruples of scaled level-$(i-1)$ codewords. Then the sequence of quadruples $(1,2^i,2^i,2^{i+1})$ does work but unfortunately, the size of the new code is only $N^2$ and this is tight. }

\[
(1), (1, 2), (2, 3), (4, 5), (8, 9), (16, 17) \ldots
\]

\[
(4, 4, 8), (8, 8, 16), (16, 16, 32), \ldots
\]


\[
(3, 3, 6), (9, 9, 18), (27, 27, 54), \ldots
\]


\begin{lemma}
There exists a sequence of numbers $a_1,\ldots, a_k$ with $k = \log_{3/2}(p)$ such that for all $\vec{v} \in \{1,2\}^k$, and all $x \in \{1,\ldots, p\}$, there exists a $y \in [5]$ and another vector $\vec{w} \in \{0,1\}^{k}$ such that $x = y+ \sum_{i=1}^k w_i\cdot v_i \cdot a_i$. That is, for all $\vec{v}$ and all $x$, $x$ can be written as the sum of numbers in a subset of $\{v_i \cdot a_i\}_{i \in [k]} \cup \{1, \ldots, 5\}$.
\end{lemma}
\begin{proof}
Consider the following sequence: $\lfloor (3/2)^j\rfloor+j/2$ for $j = 1,\ldots, \log_{3/2}(p)$. We prove by induction that all $x \in \{1,\ldots, f(m)=2(\lfloor (3/2)^{m+1}\rfloor)+m\}$ can be achieved using a $\vec{w}$ such that $w_i = 0$ for all $i > m$. \\

Base case: The claim clearly holds for $m\leq 1$. This is because the $y$ term alone suffices to write all $x \in \{1,\ldots, f(m)\}$.\\

Inductive hypothesis: Assume that the claim holds for $m$, and $m \geq 1$.\\

Inductive step: Now, consider any $x \in \{1,\ldots, f(m+1)\}$. If $x \leq f(m)$, then the inductive hypothesis immediately implies that we can write $x$ in the desired form. Now consider the case that $x > f(m)$. Then we will set $w_{m+1} = 1$, and write $x - v_{m+1}(\lfloor (3/2)^{m+1}\rfloor+m/2+1/2)$ using only the first $m$ coordinates using the inductive hypothesis. Indeed, observe that this is possible as long as $0 \leq x - v_{m+1}(\lfloor (3/2)^{m+1}\rfloor+m/2+1/2) \leq f(m)$. In particular, this holds as long the following two inequalities hold:
\begin{align*}
    0 &\leq f(m)+1 - 2(\lfloor (3/2)^{m+1}\rfloor+m/2+1/2)\\
    \Leftrightarrow f(m)+1 &\geq 2(\lfloor (3/2)^{m+1}\rfloor+m/2+1/2) \\
    \Leftrightarrow f(m) &\geq 2(\lfloor (3/2)^{m+1}\rfloor)+m.
\end{align*}
 

$$f(m+1) - (\lfloor (3/2)^{m+1}\rfloor+m/2+1/2) \leq f(m) \Leftrightarrow f(m+1) \leq \lfloor (3/2)^{m+1}\rfloor+m/2+1/2+f(m).$$

To see the first inequality, observe that it holds immediately by definition of $f(m)$. To see the second inequality, we rewrite:

\begin{align*}
    f(m+1) &= 2(\lfloor (3/2)^{m+2}\rfloor)+m+1\\
    &\leq 2\cdot( (3/2)^{m+2})+m+1\\
    &\leq 3\cdot (3/2)^{m+1}+m+1\\
    &\leq 3\cdot \lfloor (3/2)^{m+1}\rfloor +3 + m+1\\
    &\leq \lfloor (3/2)^{m+1}\rfloor+m/2+1/2
    +2(\lfloor (3/2)^{m+1}\rfloor) + m/2+1/2)\\
    &\leq \lfloor (3/2)^{m+1}\rfloor+m/2+1/2 + f(m)
\end{align*}

Observe that the last line holds as long as $m\geq 1$. 

\end{proof}

\noindent\textbf{Note:} In case we try to generalize this reasoning, observe that this proof approach works as long as $v_i \in [1,2]$ (doesn't have to be $\{1,2\}$. Could just replace the braces with brackets and the entire proof would go through.





\begin{lemma}[Triples lemma]
Let $r > 0$ be such that there exists numbers $C$ and $(a_{i, j})_{i \in [r], j \in [3]}$ satisfying $a_{i, 1} = a_{i, 2} + a_{i, 3}$ for all $i \in [r]$, and also satisfying the following: For all $x \in [p]$ and $Y \in [3]^r$, there exists 
$0 \leq c \leq C$ and $W \in \{0, 1\}^r$ such that:
\[
x = c + \sum_{i = 1}^r w_i \cdot a_{i, y_i} .
\]
Then, there exists a code with $N = 2^{2^r}$ codewords and length $O(3^r)$ that shatter all elements in $[p]$. The constant in $O(\cdot)$ depends on $C$.
\end{lemma}

The following corollary is a weaker version of the lemma that restricts attention to the case $a_{i, 1} = 2a_{i, 2} = 2a_{i, 3}$ for all $i \in [r]$. 
\begin{corollary}
Let $r > 0$ be such that there exists numbers $C$ and $(a_i)_{i \in [r]}$ satisfying the following: For all $x \in [p]$ and $Y \in [2]^r$, there exists $0 \leq c \leq C$ and $W \in \{0, 1\}^r$ such that:
\[
x = c + \sum_{i = 1}^r w_i \cdot a_i \cdot y_i .
\]
Then, there exists a code with $N = 2^{2^r}$ codewords and length $O(3^r)$ that shatter all elements in $[p]$. The constant in $O(\cdot)$ depends on $C$.
\end{corollary}

\Vnote{Old stuff below}


The following is the outline of our construction.

\begin{enumerate}
    \item The first step is constructing a base code that shatters $[k]:= \{0,\dots,k-1\}$ modulo $k$.
    \item In the second step, we do a reduction so that the new code shatters $[k]$ modulo $p$.
    \item In the final step, we blow up the code to shatter $[p]$ modulo $p$.
\end{enumerate}


\paragraph{\underline{\textbf{Step 1}}}: For this step, we currently use Alon-Alweiss construction as a black-box. For $\ell_1 > k^{3 \log \log k}$, they construct a code $\Cc_1$ over the alphabet $\Sigma_1 = [k]$ that shatters $[k]$ modulo $k$ and has $N_1\approx 2^{\ell_1}$ codewords.

\paragraph{\underline{\textbf{Step 2}}}: In this step, we construct a code $\Cc_2$ over the alphabet $\Sigma_2 = [2k]$ such that $\ell_2 = \ell_1 \cdot \log k$, $N_2 = N_1$, and shatters $[k]$ modulo $p$. The construction is as follows: for every codeword $X=(x_1,\dots,x_{\ell_1})\in \Cc_1$, where each $x_i\in [k]$, we have a corresponding codeword $X'\in \Cc_2$ such that $|X'| = |X|\cdot (\log k)$. Say $X'=(X'_0,\dots,X'_{\log k-1})$. We set $X'_0 = X$. For $1\le i<\log k$, we set $(X'_i)_j = x_j$ if $i$-th bit of $x_j$ is $1$. Else, we set $(X'_i)_j = x_j+k$. We now argue the correctness. Consider any two codewords $X,Y\in \Cc_1$. Let $X',Y'$ be their corresponding codewords in $\Cc_2$. For every $g\in [k]$, $\exists j$ such that $x_j - y_j = g \mod k$. If $x_j\ge y_j$, then $x_j-y_j = g \mod p$. Else if $x_j<y_j$, then there exists $i$ such that the $i$-th bit of $x_j$ is 0, and the $i$-th bit of $y_j$ is $1$. Then $(X'_i)_j-(Y'_i)_j \mod p = x_i+k-y_i \mod p = g \mod p$.

\paragraph{\underline{\textbf{Step 3}}}: Finally, we construct a code $\Cc_3$ over $\Sigma_3 = [p]$ such that $\ell_3 = \frac{p\log p}{k}\cdot \ell_2$, $N_3=N_2$, and shatters $[p]$ modulo $p$. In order to construct this code, we need the following fact: for every $k<p$,  there exists $S\subseteq [p]$ such that $|S|\le \frac{p\log p}{k}$ and for every $g\in [p]$, $\exists i\in [k], j\in S$ such that $i\cdot j = g$.  %\Vnote{For this step, we can replace the shattered set $[k]$ with any set of size $k$, and the previous fact still holds.} 
In order to prove the fact, choose $S$ to be a random subset of $\frac{p\log p}{k}$ elements from $[p]$. For any $g\in \mathbb{Z}_{p}^*$, probability that there is no $j\in S$ such that $i\cdot j = g$ for some $i\in [k]$ is at most $(1-\frac{k}{p})^\frac{p\log p}{k}<1/p$. Applying the union bound over all $g$, we conclude that the probability that there exists such a $g$ is strictly less than $1$, and hence there exists some $S$ such that $|S|\le \frac{p\log p}{k}$ and for every $g\in [p]$, $\exists i\in [k], j\in S$ such that $i\cdot j = g$.
For every codeword $X'\in \Cc_2$, we construct a corresponding codeword $X''\in \Cc_3$ where $X'' = (s_1\cdot X', \dots, s_{|S|}\cdot X')$, where $s_1,\dots,s_{|S|}$ are the elements of $S$.


\paragraph{\underline{\textbf{Putting them together}}}:
If we set $k=p^{\frac{1}{3\log \log p}}$ and $\ell_1 = p\log p$, then $N_3=N_1\approx 2^{\ell_1}= p^p$. Putting all the above steps together, we get
\[
\ell_3 = \ell_1 \cdot \frac{p\log p\cdot \log k}{k} = p^2 (\log p)^2 \cdot \frac{\log k}{k} = p^{2-\frac{1}{3\log \log p}}\cdot \frac{(\log p)^3}{3\log \log p} = o(p^2) \, .
\]

\paragraph{\underline{\textbf{The bound on $\ell_3$ for general $N$}}}
For $N\le 2^{p^{3\log \log P}}$, we have  $(\log N)^{\frac{1}{3\log\log\log N}}\le p$. In this case, we can set $k=(\log N)^{\frac{1}{3\log\log\log N}}$ and $\ell_1=\log N$, then $N_3=N_1\approx 2^{\ell_1}= N$. Putting all the above steps together, we get
\[
\ell_3 = \ell_1 \cdot \frac{p\log p\cdot \log k}{k} = p\log p \cdot (\log N)^{1-\frac{1}{3\log \log\log N}}\cdot \frac{\log \log N}{3\log\log\log N} \, .
\]
In particular, $\AAM(p,N) \lesssim p\log p \cdot (\log N)^{1-\frac{1}{3\log \log\log N}}\cdot \frac{\log \log N}{3\log\log\log N}$.
\begin{remark}[The bound in \cite{AA20} ]
For $N\ge  (2-\frac{1}{\log p})^{p^{5\log \log p}}$, it follows from \cref{thm:aa20} that $\AAM(p,N)\le \log_{\left(2-\frac{1}{\log p}\right)}N$.
\end{remark}
